Automatic extraction of cause-effect-relations from requirements artifacts

Background: The detection and extraction of causality from natural language sentences have shown great potential in various fields of application. The field of requirements engineering is eligible for multiple reasons: (1) requirements artifacts are primarily written in natural language, (2) causal sentences convey essential context about the subject of requirements, and (3) extracted and formalized causality relations are usable for a (semi-)automatic translation into further artifacts, such as test cases. Objective: We aim at understanding the value of interactive causality extraction based on syntactic criteria for the context of requirements engineering. Method: We developed a prototype of a system for automatic causality extraction and evaluate it by applying it to a set of publicly available requirements artifacts, determining whether the automatic extraction reduces the manual effort of requirements formalization. Result: During the evaluation we analyzed 4457 natural language sentences from 18 requirements documents, 558 of which were causal (12.52%). The best evaluation of a requirements document provided an automatic extraction of 48.57% cause-effect graphs on average, which demonstrates the feasibility of the approach. Limitation: The feasibility of the approach has been proven in theory but lacks exploration of being scaled up for practical use. Evaluating the applicability of the automatic causality extraction for a requirements engineer is left for future research. Conclusion: A syntactic approach for causality extraction is viable for the context of requirements engineering and can aid a pipeline towards an automatic generation of further artifacts from requirements artifacts.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> chapters/04_evaluation.tex <==
\section{Evaluation}
\label{section:eval}

The purpose of the following preliminary study is to prove the feasibility of the causality recognition and phrase extraction method based on syntactic similarities. For this, we use the cerec system as described in Section~\ref{section:impl} with lexical constraints and train a set of requirements artifacts containing natural language sentences.

\subsection{Design}
A publicly available dataset \textit{A} containing requirements artifacts $a \in A$ was selected for the evaluation of the implemented approach. The obvious choice is using the SemEval 2010 Task 8 dataset \cite{hendrickx2010semeval}, which is often used for the evaluation of causality extraction approaches because causal sentences are already annotated. However, the annotated causal phrases are limited to pairs of events, predominantly two nouns, in semantically causal relation. Our proposed algorithm works on the dataset, but evaluating its effectiveness by detecting causally related noun-pairs defeats the purpose of tailoring the proposed algorithm to requirements engineering. Instead we used the PURE dataset of public requirements documents \cite{ferrari2017pure} and manually annotated 13 of the 18 available artifacts for evaluation. Only full natural language sentences were regarded, as these are subject to our approach. The 13 datasets collectively contained 2373 sentences, 282 of which (11.88\%) are causal. \newline
To assess our approach we formulated the following research questions:
\begin{itemize}
    \item \textbf{RQ1}: How effective is the algorithm in automatically detecting and extracting causal relations in a single requirements document?
    \item \textbf{RQ2}: How effective is the algorithm in automatically detecting and extracting causal relations in a single requirements document with previous training?
    %\item \textbf{RQ3}: How much do lexical constraints contribute to the effectiveness of the algorithm in detecting and extracting causal relations?
\end{itemize}
To evaluate the effectiveness of the algorithm, the system will be \textit{fully trained}: a dataset will be randomly ordered and provided to the system sentence by sentence in a \textit{training} operation. The system will perform this operation and evaluate the process with one of the following flags:
\begin{itemize}
    \item recognition successful (rec+): a causal sentence is accepted by an existing pattern and the causal relation has been extracted accordingly
    \item discarding successful (disc+): a non-causal sentence has not been accepted by an existing pattern
    \item creation successful (crea+): a causal sentence has not been accepted by an existing pattern, but a new pattern has been established that covers this sentence
    \item creation failed (crea-): a causal sentence has not been accepted by an existing pattern and no new pattern could be established to cover this sentence
    \item specification successful (spec+): a sentence has been compliant to an existing pattern, but not applicable to its phrase extraction method, so the pattern has been specified to restore the principles of maintenance
    \item specification failed (spec-): a sentence has been compliant to an existing pattern, but not applicable to its phrase extraction method, and the specification failed to differentiate the sentence from the pattern
\end{itemize}
The six flags compose the containing set \textit{F}:
$$F = \{rec+, disc+, crea+, crea-, spec+, spec-\}$$
The full training process simulates the expected user interaction with the system: while writing natural language sentences of a requirements document, the system attempts to detect a causality in every sentence upon its completion. If a causal sentence is recognized and the causal phrases are extracted correctly, the process is flagged as \textit{rec+}. If the causal sentence is not recognized, the interacting user can manually select the cause- and effect-phrase of the sentence and train the system by providing the causal relation alongside the sentence. This information is used for a training process and upon success will generate a new pattern, which flags the process as \textit{crea+}. Should this process fail for any reason, the process is flagged as \textit{crea-}. Should the algorithm detect the causality of a sentence but extract a cause- and effect-expression that does not align with the user's perception of the conveyed causality, he can manually correct the cause- and effect-expression of the sentence, which will be used for a specification process as described in Section~\ref{impl:maintenance:specification}, as the sentence is seemingly compliant to a pattern but not applicable by its phrase extraction method. \newline
If the specification succeeds, the run is flagged as \textit{spec+} -- otherwise \textit{spec-}. If a non-causal sentence is non-compliant to any pattern, the sentence is correctly discarded, which is flagged as \textit{disc+}. If the non-causal sentence is wrongfully compliant to a pattern, a specification algorithm has to be performed again. The overall training process is illustrated in Figure~\ref{fig:process:training}. Here processes are written in round-edge boxes and can result in success or failure. \newline 
\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{images/processes/training_process.pdf}
    \caption{Decision diagram on the training process}
    \label{fig:process:training}
\end{figure*}

\subsection{Measures}
The distribution of occurring flags allows to evaluate the effectiveness of the algorithm. We introduce the notation $n_{f}(a)$ as the number of training processes of the artifact $a \in A$ tagged with a specific flag $f \in F$. Three measures evaluate training the cerec system with all sentences of a requirements artifact. The \textit{trained correct decision rate} of an artifact, tcdr(a) in Equation~\ref{eq:1}, calculates the amount of sentences correctly handled by the system at its current state of training. A training process evaluated as rec+ or disc+ means that the system handled a sentence correctly without further intervention. This rate represents the degree of automation, to which the sentences are processed correctly and without manual effort.
\begin{equation} \label{eq:1}
    tcdr(a) = \frac{n_{rec+}(a) + n_{disc+}(a)}{\sum_{f \in F}^{} n_f(a)}
\end{equation}
The \textit{active learning correct decision rate} of an artifact, alcdr(a) in Equation~\ref{eq:2}, calculates the number of sentences correctly handled by the system overall. It extends the trained correct decision rate as it also takes into account training processes evaluated as spec+ or crea+, which require further manual effort. This rate represents the overall capability of handling sentences correctly.
\begin{equation} \label{eq:2}
    alcdr(a) = \frac{n_{rec+}(a) + n_{disc+}(a) + n_{crea+}(a) + n_{spec+}(a)}{\sum_{f \in F}^{} n_f(a)}
\end{equation}
The \textit{recognition rate} of an artifact, recr(a) in Equation~\ref{eq:3}, calculates how many of the causal sentences have been correctly recognized and the causality extracted. This measure assesses to which degree the system automates the extraction of causal phrases. Given that $n_{c}(a)$ represents the number of causal sentences in the artifact a, the recognition rate of an artifact $a \in A$ is:
\begin{equation} \label{eq:3}
    recr(a) = \frac{n_{rec+}(a)}{n_{c}(a)}
\end{equation}

\subsection{RQ1: Effectiveness of the algorithm without training}
The study of RQ1 simulates the use of the system in an environment without any previous training, which means that no causality patterns exist at the start of the evaluation. Table~\ref{tab:RQ1_values} shows the results of the measures on the requirements artifacts, on which the evaluation has been performed. The mean recognition rate is 16.02\%. The overall recall $\frac{\sum_{a \in A} n_{rec+}(a)}{\sum_{a \int A} n_{causal}(a)}$ is 22.51\%, more accurately representing the recognition rate, while the overall precision is 54.76\% and the F-measure 31.9\%.

\begin{table}
    \centering
    \begin{tabular}{|l|r|r|r|r|r|} \hline
        \textbf{Artifact a} & \textbf{n(a)} & \textbf{n\textsubscript{c}(a)} & \textbf{alcdr(a)} & \textbf{tcdr(a)} & \textbf{recr(a)} \\ \hline
        blitdraft & 67 & 19 & 100.00\% & 74.92\% & 17.89\% \\ \hline
        cctns & 183 & 28 & 99.45\% & 85.03\% & 10.71\% \\ \hline
        dii & 40 & 1 & 100.00\% & 97.50\% & 0.00\% \\ \hline
        eirene & 520 & 66 & 98.15\% & 89.27\% & 21.21\% \\ \hline
        ermts & 223 & 42 & 99.46\% & 86.37\% & 31.42\% \\ \hline
        gammaj & 203 & 3 & 100.00\% & 98.52\% & 0.00\% \\ \hline
        gemini & 392 & 12 & 99.23\% & 96.83\% & 0.00\% \\ \hline
        getreal & 99 & 2 & 100.00\% & 97.98\% & 0.00\% \\ \hline
        keepass & 191 & 46 & 99.47\% & 80.21\% & 22.60\% \\ \hline
        microcare & 39 & 8 & 100.00\% & 77.44\% & 0.00\% \\ \hline
        peering & 131 & 13 & 96.94\% & 89.16\% & 3.07\% \\ \hline
        qheadache & 107 & 14 & 99.81\% & 93.46\% & 51.42\% \\ \hline
        themas & 178 & 28 & 98.87\% & 91.35\% & 50.00\% \\ \hline
    \end{tabular}
    \caption{Results for automatic causality extraction without previous training}
    \label{tab:RQ1_values}
\end{table}

The evaluation shows high active learning correct decision rate (alcdr), translating to a good handling rate of sentences in general. The negative influence on this measure mainly stems from issues caused by the NLP pipeline, where for example unknown acronyms at the end of the sentence cause problems with sentence formalization. The overall high trained correct decision rate (tcdr) indicates an high degree of automation, to which sentences are handled by the system without further effort. However, the actual benefit of the causality extraction is most precisely represented by the recognition rate (recr), since discarding non-causal sentences is positive for the tcdr, but does not generate any value from the sentences. \newline 
Two major insights can be derived from the results of this study: first, the overall number of causal sentences is directly proportionate to the recognition rate. The recall of all artifacts with 13 or less causal sentences is 3.08\%, while the recall of all artifacts with more than 13 causal sentences is 26.83\%. The relation between number of causal sentences and recognition rate is due to the nature of the machine learning approach, where an increased number of training data provides more patterns, which the system can learn and reuse for detection and extraction later. \newline
The second insight is that also the number of causal linguistic patterns used is directly proportionate to the recognition rate. This can be observed when comparing the results of the two artifacts \textit{peering} and \textit{qheadache} with each other: even though they contain almost the same amount of causal sentences, qheadache presents a significantly higher recognition rate. Investigating the resulting patterns yields that the repeated use of a causal linguistic pattern "If <S>, <NP> <VP>." generated a pattern with the signature shown in Figure~\ref{fig:signature_qheadache}. 
\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{images/evaluation/qheadache_patternSignature.pdf}
    \caption{Signature of pattern no1 generated from the \textit{qheadache} requirements artifact}
    \label{fig:signature_qheadache}
\end{figure}
Once the pattern was established by manually annotating the first occurrence of this linguistic pattern, all comparable sentences were compliant and also applicable by the generated phrase extraction method. Sentences like "If the file was correctly updated, there is no output." and "If the game is not saved, a dialog box is displayed that asks to the player if he wants to save the game." are compliant to the pattern and the phrase extraction method generated the correct cause- and effect-phrase, therefore successfully automatizing the causality recognition and extracion for these sentences. \newline
The consequence of the two insights are discussed in the conclusion.

\subsection{RQ2: Effectiveness of the algorithm with previous training}
The study of RQ2 simulates the use of the system in an environment with previous training, which means that causality patterns already exist at the start of the evaluation. To simulate this, each of the requirements artifacts were tested like in RQ1, but only after the system has been previously trained with all other artifacts beforehand, effectively starting the training with all patterns extracted from the other artifacts. The results are shown in Table~\ref{tab:RQ2_values}.

\begin{table}
    \centering
    \begin{tabular}{|l|r|r|r|r|r|} \hline
        \textbf{Artifact a} & \textbf{n(a)} & \textbf{n\textsubscript{c}(a)} & \textbf{alcdr(a)} & \textbf{tcdr(a)} & \textbf{recr(a)} \\ \hline
        blitdraft & 67 & 19 & 100.00\% & 74.93\% & 11.57\% \\ \hline
        cctns & 183 & 28 & 99.34\% & 86.89\% & 14.28\% \\ \hline
        dii & 40 & 1 & 100.00\% & 97.50\% & 0.00\% \\ \hline
        eirene & 520 & 66 & 98.15\% & 90.15\% & 23.33\% \\ \hline
        ermts & 223 & 42 & 99.55\% & 83.05\% & 11.90\% \\ \hline
        gammaj & 203 & 3 & 100.00\% & 98.42\% & 33.33\% \\ \hline
        gemini & 392 & 12 & 99.23\% & 96.94\% & 11.66\% \\ \hline
        getreal & 99 & 2 & 100.00\% & 97.98\% & 0.00\% \\ \hline
        keepass & 191 & 46 & 99.27\% & 78.53\% & 13.04\% \\ \hline
        microcare & 39 & 8 & 100.00\% & 82.05\% & 12.50\% \\ \hline
        peering & 131 & 13 & 96.95\% & 90.53\% & 4.61\% \\ \hline
        qheadache & 107 & 14 & 98.69\% & 91.59\% & 35.71\% \\ \hline
        themas & 178 & 28 & 98.88\% & 91.80\% & 47.85\% \\ \hline
    \end{tabular}
    \caption{Results for automatic causality extraction with previous training}
    \label{tab:RQ2_values}
\end{table}

%It becomes obvious that the recognition rate has not increased, but rather decreased in general: though the mean recognition rate is 16.91\%, the weighted mean recognition rate is now 19.5\%, which means that even though some artifacts now have higher recognition rates, the overall number of recognized causal sentences has dropped. There is also no significant increase in the trained correct decision rate, therefore no improvement of automation. \newline
%The opposite effect might be expected, since already existing patterns should provide a larger basis for causality detection. Only artifacts with an overall low number of causal sentences benefit from the previous training with a weighted mean recognitionrate of 7.7\%, while artifacts with a high number of causal sentences have a reduced weighted mean recognition rate of 21.4\%. \newline
%Two reasons are identified for this effect: first, the sets of linguistic patterns used in each requirements artifact only rarely intersect. Linguistic patterns for causal sentences differ greatly from artifact to artifact, which mitigates providing valuable patterns for other artifacts. \newline
%Secondly, the previous existence of patterns, which are close to patterns used in an artifact so that they are compliant to the signature, but not similar enough to be applicable by the phrase extraction method, will result in a lot of false compliance. Sentences being compliant to patterns but not applicable by their phrase extraction method, require a specification described in Section~\ref{impl:maintenance:specification}, which only works by manually providing the correct cause- and effect-phrase. This manual effort counteracts the attempt of automatizing causality extraction. The reason for this relation might be the lack of maturity of the system, which does not yet cope well with large amounts of different sources and diminishes the benefits of large and multi-source training data. \newline
Evaluating the system with previous training results in a precision of 68.4\%, a recall of 21.4\% and an overall F-measure of 32.6\%. Compared to the results of RQ1, the effect of previous training on the algorithm is not entirely positive: the precision has increased, which means that more of the compliant sentences were actually causal and recognized successfully. This comes at the cost of a decreased recall, which means that less sentences were compliant to patterns in general. In total these changes result in a roughly similar F-measure compared to RQ1. \newline
The training beforehand established a large set of patterns based on a corpus vastly outnumbering the sentences contained by the artifact under test. These patterns have undergone a multitude of specification processes as described in Section~\ref{impl:maintenance:specification}, which accounts for the increase in precision of the overall algorithm. On the other hand, the increased specificity of patterns causes less sentences of the artifact under test to be compliant, decreasing the recall. The evaluation of RQ2 shows that the system does not yet profit from an increased beforehand training, which leaves room for improving the scalability of the approach. \newline
It is worth mentioning that the lack of improvement in recall when performing RQ2 in contrast to RQ1 is further rooted in the fact that the evaluation was performed on a very heterogeneous set of requirements, written by different authors in different domains. A common template or guideline for writing requirements was most probably absent, which would have increased the similarity of linguistic causality patterns and therefore the recognition rate. The evaluation was from this perspective performed under worst-case conditions with artifacts that are biased against a learning system that relies on consistency and patterned expressions, which mitigates the benefit from previous training.

==> chapters/06_logics.tex <==
\section{Logics}
This chapter is just a draft for logical expressions of concepts

\subsection{Predicates}
\begin{center}
    \begin{tabular}{|l|l|} \hline
        P & explanation \\ \hline
        sen(x) & x is a sentence \\ \hline
        c(x) & x is causal (coveys a causal relation) \\ \hline
        str(x) & x is a graphical structure \\ \hline
        so(x, y) & y is the structure associated with x \\ \hline
        sub(x, y) & y is a subtree of x \\ \hline
        seq(x, z) & x is equivalent to y \\ \hline
        p(x) & x is a pattern \\ \hline
        cmp(x, y) & y is compliant to x \\ \hline
        ex(x) & x is an extraction algorithm \\ \hline
        ceg(x) & x is an cause effect graph \\ \hline
        co(x, y) & y describes the causal relation of x \\ \hline
        % & \\ \hline
    \end{tabular}
\end{center}

\subsection{Formulas}
For every causal sentence there is a cause-effect-graph that describes the causal relation which that sentence conveys.
\begin{equation}
    \forall s (sen(s) \land c(s)) \rightarrow (\exists c ( ceg(c) \land co(s, c)))
\end{equation} 
Every pattern, which is compliant to sentence $s_1$, is compliant to every sentence $s_2$ if the structure of both sentences is equivalent
\begin{equation}
    \forall p \forall s_1 (p(p) \land sen(s_1) \land cmp(p, s_1) \rightarrow \forall s_2, str_1, str_2 (sen(s_2) \land so(s_1, str_1) \land so(s_2, str_2) \land seq(str_1, str_2) \rightarrow cmp(p, s_2) ))
\end{equation}
Every pattern has an associated structure.
\begin{equation}
    \forall p (p(p) \rightarrow \exists s_p (str(s_p) \land so(p, s_p))
\end{equation}
The structure associated with a pattern is a subtree of each sentence, which is compliant to the pattern
\begin{equation}
    \forall p \exists s_p (p(p) \land str(str_p) \land so(p, str_p) \rightarrow \forall s \exists str_s (sen(s) \land str(str_s) \land so(s, str_s) \rightarrow (cmp(p, s) \iff sub(str_s, str_p))))
\end{equation}
